A QCD analysis of ZEUS diffractive data

ZEUS inclusive diffractive cross-section measurements have been used in a DGLAP next-to-leading-order QCD analysis to extract the diffractive parton distribution functions. Data on diffractive dijet production in deep inelastic scattering have also been included to costrain the gluon density. Predictions based on the extracted parton densities are compared to diffractive charm and dijet photoproduction data.

==> paper-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
%\ifMartex
%  \bibliographystyle{/bologna/user2/arneodo/l4z/BiBTeX/bst/l4z_default}
%\else
  \bibliographystyle{l4z_default}
%\fi
\fi
\ifzdrftbst
  \bibliographystyle{/bologna/user2/arneodo/l4z/BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{/bologna/user2/arneodo/l4z/BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{l4z_pl}
\fi
{\raggedright
%\ifMartex
	\bibliography{/bologna/user2/arneodo/l4z/BiBTeX/bib/l4z_zeus,paper}}
%\else
	\bibliography{l4z_zeus,paper}
%\fi
% \bibliography{l4z_zeus}
}
\vfill\eject

